Finitely Presentable Higher-Dimensional Automata and the Irrationality of Process Replication

Higher-dimensional automata (HDA) are a formalism to faithfully model the behaviour of concurrent systems. For ordinary automata, there is a correspondence between regular expressions, regular languages and finite automata, which provides a powerful link between algebraic proofs and operational behaviour. It has been shown by Fahrenberg et al. that finite HDA correspond with interfaced interval pomset languages generated by sequential and parallel composition and non-empty iteration, and thereby to a variant of Kleene algebras (KA) with parallel composition. It is known that this correspondence cannot be extended to concurrent KA, which additionally have process replication. An alternative to finite HDA are locally finite HDA, in which every state can only reach finitely many other states, and finitely branching HDA. In this paper, we show that both classes of HDA are closed under process replication and thus models of concurrent KA. To achieve this, we prove that the category of HDA is locally finitely presentable, where the finite HDA generate all other HDA. We then prove that this has the unfortunate side-effect that all HDA are locally finite, which means that the correspondence with concurrent KA trivialises. Similarly, we also show that, even though finitely branching HDA are closed under process replication, the resulting HDA necessarily have infinitely many initial states.

==> content/fp-hda-backup.tex <==
\section{Rational HDA}
\label{sec:fp-hda}

\todo[inline]{Due to the fact that being able to canonically express every HDA as the filtered colimit of a diagram of finite HDA is extremely useful for some proofs (for example theorem \ref{languages-tensor}) it might be best to place this section somewhere else. This might be difficult depending on what we cover in subsection \ref{sec:replication}, in which case we might split this section? Alternatively we can use theorems before proving them, and proving them here or in the appendix.}

\subsection{Filtered Colimits and Compact HDA}
\label{sec:compact-hda}

\todo[inline]{In this subsection we prove that the category of HDA is locally finitely presentable and that a HDA is compact if and only if it is finite.}
\begin{definition}
A representable precubical set is a precubical set that is naturally isomorphic to the Yoneda embedding $\Yo_{U} = \Cube(-, U)$ for some object $U$ in $\Cube$.
\end{definition}
For every lo-set $V$ in $\Cube$ the set $\Cube(V,U)$ is the collection of all coface maps $V\to U$. Note that for each $U$ there only exist a finite amount of these lo-sets $V$ where $\Cube(V,U)\not=\emptyset$, and between each $V$ and $U$ there only exist a finite amount of coface maps. Therefore the representable precubical sets are finite.
\todo[inline]{Explain with an example? For example let's say we have $U=\left(a\dr b\right)$. Then by definition of $\Cube$ the only lo-sets that have coface maps with target $U$ are $\varepsilon$, $(a)$, $(b)$ and $\left(a\dr b\right)$ itself.}
\todo[inline]{Do we want theorems (or strong explanations) for why the above about the coface maps is true?}
\todo[inline]{Now that I understand the definition of compactness a bit better I think there might be a much easier way to prove that compactness is the same as finiteness for both precubical sets and HDA.}
\begin{lemma} \label{filtered-finite-set}
Let $D$ be a filtered category and suppose that we have a finite set of objects $\left\{d_1,d_2,...,d_n\right\}$ in $D$. Then there exists an object $d\in D$ and a finite set of morphisms $\left\{f_1,f_2,...,f_n\right\}$ with $f_i:d_i\to d$.
\end{lemma}
\begin{proof}
\todo[inline]{Maybe too trivial to write down as a lemma? For each pair $d_i,d_j$ there exists a $d_{i,j}$ and morphisms $g_i:d_i\to d_{i,j}$ and $g_j:d_j\to d_{i,j}$. This then gives us a set of objects of size $n-1$, which by induction eventually gives us the object $d\in D$ with the required morphisms.}
\end{proof}
\begin{lemma} \label{HDA-diagram-image}
Let $X$ be a finite HDA, let $F:D\to\HDA$ be a filtered diagram with the colimit $(Y,\phi)$ and let $f:X\to Y$ be a HDA map. Then there exists a $d\in D$ such that there exists a HDA map $g:X\to F(d)$ with $\phi(d)\circ g=f$.
\end{lemma}
\begin{proof}
Since $X$ is finite the image $f(X)=\bigsqcup_{U\in\Cube}f[U]\circ X[U]$ is finite as well. For each $U\in\Cube$ and each $y\in Y[U]$ for which there exists a $x\in X[U]$ with $f[U](x)=y$ there exists a $d_z\in D$ and a $z\in F(d)[U]$ such that $\phi_{d_z}[U](z)=y$ and for which we have $z\in \sCells{F\left(d_z\right)}\iff y\in\sCells{Y}$ and $z\in \aCells{F\left(d_z\right)}\iff y\in\aCells{Y}$. Then because of lemma \ref{filtered-finite-set} there exists a $d\in D$ such that for each $U\in\Cube$ and each $x\in X[U]$ there exists a $z\in F(d)[U]$ with $f[U](x)=\phi_d[U](z)$ with $x\in\sCells{X}\implies z\in \sCells{F\left(d_z\right)}$ and $x\in\aCells{X}\implies z\in \aCells{F\left(d_z\right)}$.

Because $X$ is finite this gives us a finite set of these elements of $F(d)$. Using the properties of filtered categories we get that there exists a $d\in D$ such that this finite set is closed under the face maps. Then based on this finite set there exists a unique HDA map $g:X\to F(d)$ with $\phi_d\circ g=f$.
\end{proof}
\todo[inline]{The proof is a bit messy and possibly doesn't explain things thoroughly enough.}
\todo[inline]{There are a few things that could possibly benefit from referencing a lemma:

(1): For each $y\in Y[U]$ there exists a $d_z\in D$ and a $z\in F\left(d_z\right)[U]$ such that $\phi_{d_z}[U](z)=y$, $z\in \sCells{F\left(d_z\right)}\iff y\in\sCells{Y}$ and $z\in \aCells{F\left(d_z\right)}\iff y\in\aCells{Y}$.

(2): \textit{"Using the properties of filtered categories we get that there exists a $d\in D$ such that this finite set is closed under the face maps."} might need something more. Suppose that for certain $U,V\in\Cube$, $x_1\in X[U]$, $x_2\in X[V]$, $\nu\in\{0,1\}$ and $A=U\backslash V$ we have $\delta^{\nu}_A\left(x_1\right)=x_2$. Also suppose that in our finite set we have $f[U]\left(x_1\right)=\phi_d[U]\left(z_1\right)$ and $f[V]\left(x_2\right)=\phi_d[V]\left(z_2\right)$ but also $\delta^{\nu}_A\left(z_1\right)\not=z_2$. Then because $\phi_d[V]\circ \delta^{\nu}_A\left(z_1\right)=\phi_d[V]\left(z_2\right)$ we have $\delta^{\nu}_A\left(z_1\right)\sim z_2$ which because $D$ is filtered means that there exists an object $e\in D$ and a $h:d\to e$ such that $F(h)\circ\delta^{\nu}_A\left(z_1\right)=F(h)\left(z_2\right)$. Since our set of elements is finite we can repeat this process until we get an $F(d)$ where the finite set is closed under the face maps.

(3): \textit{"Then based on this finite set there exists a unique HDA map $g:X\to F(d)$ with $\phi_d\circ g=f$.}" again feels a little to quick. However the way we found our $F(d)$ and defined our finite set perfectly defined what the image of the map $g:X\to F(d)$ would need to be. For each $x\in X[U]$ we have found a $z\in F(d)[U]$ (that isn't necessarily unique) such that $x\in\sCells{X}\implies z\in\sCells{F(d)}$, $x\in\aCells{X}\implies z\in\aCells{F(d)}$ and such that for all face maps $\delta^{\nu}_A$ the element $\delta^{\nu}_A(x)$ is mapped to the element $\delta^{\nu}_A(z)$.}
\todo[inline]{Note that the HDA map $g:X\to F(d)$ might not be unique.}
\todo[inline]{Maybe we want the statement to be the following instead: Let $X$ be a HDA, let $F:D\to\HDA$ be a filtered diagram with the colimit $(Y,\phi)$ and let $f:X\to Y$ be a HDA map. If $X$ is a finite HDA then the HDA map $f:X\to Y$ factors through some $F(d)$.}
\begin{lemma} \label{finite-sim-maps}
Let $X$ be a finite HDA, let $F:D\to\HDA$ be a filtered diagram with the colimit $(Y,\phi)$ and let $f_1,f_2:X\to F(d)$ be HDA maps for a certain $d\in D$. Then we have $\phi_d\circ f_1=\phi_d\circ f_2$ if and only if there exists a $e\in D$ and a morphism $g:d\to e$ such that $F(g)\circ f_1=F(g)\circ f_2$.
\end{lemma}
\begin{proof}
Suppose that there exists a $e\in D$ and a morphism $g:d\to e$ such that $F(g)\circ f_1=F(g)\circ f_2$. Then we have $\phi_e\circ F(g)\circ f_1=\phi_e\circ F(g)\circ f_2$ which automatically gives us $\phi_d\circ f_1=\phi_d\circ f_2$, since for all $U\in\Cube$ and all $x\in X[U]$ we have
\[
\phi_d\circ f_1[U](x)=\phi_e\circ F(g)\circ f_1[U](x)=\phi_e\circ F(g)\circ f_2[U](x)=\phi_d\circ f_2[U](x)
\]
Suppose that we have $\phi_d\circ f_1=\phi_d\circ f_2$. Then for all $U\in\Cube$ and all $x\in X[U]$ we have $\phi_d\circ f_1[U](x)=\phi_d\circ f_2[U](x)$. Because of theorem \ref{colimit-sim-iff} this is true if and only if there exist $e_x\in D$ and morphisms $g_1,g_2:d\to e_x$ such that $F\left(g_1\right)\circ f_1[U](x)=F\left(g_2\right)\circ f_2[U](x)$. Because $D$ is filtered there exists a $e_x'\in D$ and a $h:e_x\to e_x'$ such that $h\circ g_1=h\circ g_2$. For the sake of convenience we say that for all $U\in\Cube$ and all $x\in X[U]$ there exists a $e_x\in D$ and a $g_x:d\to e_x$ such that $F\left(g_x\right)\circ f_1[U](x)=F\left(g_x\right)\circ f_2[U](x)$.

Since $X$ is finite this gives us only a finite amount of $e_x\in D$. Therefore there exists a $e\in D$ and morphisms $h_x:e_x\to e$ for each $U\in \Cube$ and each $x\in X[U]$. This gives us the morphisms $h_x\circ g_x:d\to e$ which then because of $D$ being a filtered category gives us a morphism $h:e\to e'$ such that $h\circ h_x\circ g_x=h\circ h_y\circ g_y$ for all $U,V\in\Cube$ and all $x\in X[U]$, $y\in X[V]$.

Therefore for all $U\in\Cube$ and all $x\in X[U]$ we have a morphism $h\circ h_x\circ g_x:d\to e'$. This morphism is the same for all $U\in \Cube$ or $x\in X[U]$. Renaming $e'$ to $e$ and $h\circ h_x\circ g_x$ to $g$ gives us the required morphism.
\end{proof}
\begin{theorem}
Every finite HDA or finite precubical set is compact.
\end{theorem}
\begin{proof}
Let $\HDATup{X}$ be a finite HDA and let $F:D\to\HDA$ be a filtered diagram with the colimit $(Y,\phi)$. This gives us the filtered diagram $\text{Hom}\left(X,F(-)\right):D\to\SetC$ with the filtered colimit $\left(\colim_{d\in D}\text{Hom}\left(X,F(d)\right),\Phi\right)$. By definition $\text{Hom}(X,Y)$ is a cocone of $\text{Hom}\left(X,F(-)\right)$ with the injection maps $\text{Hom}(X,\phi)$ which gives us the unique morphism $q:\colim_{d\in D}\text{Hom}\left(X,F(d)\right)\to\text{Hom}(X,Y)$. For all $d\in D$ we have $q\circ\Phi_d=\text{Hom}\left(X,\phi_d\right)$.

We want to prove that this $q$ is an isomorphism. Suppose that we have $f\in\text{Hom}(X,Y)$. Then lemma \ref{HDA-diagram-image} gives us that there exists a $d\in D$ and a $g\in\text{Hom}\left(X,F(d)\right)$ with $\phi_d\circ g=f$ and therefore $f=\text{Hom}\left(X,\phi_d\right)(g)=q\circ\Phi_d(g)$. This means that $q$ is surjective.

Let $f_1,f_2\in\colim_{d\in D}\text{Hom}\left(X,F(d)\right)$. Then there exist $d_1,d_2\in D$, $g_1\in\text{Hom}\left(X,F\left(d_1\right)\right)$ and $g_2\in\text{Hom}\left(X,F\left(d_2\right)\right)$ with $\Phi_{d_1}\circ g_1=f_1$ and $\Phi_{d_2}\circ g_2=f_2$. Because $D$ is a filtered category there exists a $d\in D$ and morphisms $h_1:d_1\to d$ and $h_2:d_2\to d$ such that $\Phi_d\circ F\left(h_1\right)\circ g_1=f_1$ and $\Phi_d\circ F\left(h_2\right)\circ g_2=f_2$.

This gives us that for all $f_1,f_2\in\colim_{d\in D}\text{Hom}\left(X,F(d)\right)$ there exists a $d\in D$ and HDA maps $g_1,g_2\in\text{Hom}\left(X,F(d)\right)$ with $\Phi_d\circ g_1=f_1$ and $\Phi_d\circ g_2=f_2$. Suppose that $q\circ f_1=q\circ f_2$. This gives us $\phi_d\circ g_1=\phi_d\circ g_2$. Then we can use lemma \ref{finite-sim-maps} to give us an object $e\in D$ and a morphism $h:d\to e$ with $F(h)\circ g_1=F(h)\circ g_2$. By definition this then gives us that $\Phi_d\circ g_1=\Phi_d\circ g_2$ and therefore $f_1=f_2$, which means that $q$ is injective as well.
\todo[inline]{Do we still want to prove this for precubical sets? It wouldn't be too hard but it might not really be necessary. Note that the theorem statement might need to be changed.}
\end{proof}
\begin{theorem}
All representable precubical sets are compact.
\end{theorem}
\begin{proof}
Let $X$ be a representable precubical set. Then there exists an object $U$ in $\Cube$ such that $X\cong\Cube(-,U)$. Suppose that $F:D\to\presheaf{\Cube}$ is a small filtered diagram. The Yoneda lemma/Yoneda reduction then gives us
\[
\colim_{d\in D}\left(\text{Hom}\left(X,F(d)\right)\right)\cong\colim_{d\in D}\left(\text{Hom}\left(\Cube(-,U),F(d)\right)\right)\cong\colim_{d\in D}\left(F(d)(U)\right)
\]
\[
\text{Hom}\left(X,\colim_{d\in D}F(d)\right)\cong\text{Hom}\left(\Cube(-,U),\colim_{d\in D}F(d)\right)\cong\left(\colim_{d\in D}F(d)\right)(U)
\]
And we get $\colim_{d\in D}\left(F(d)(U)\right)\cong\left(\colim_{d\in D}F(d)\right)(U)$ from proposition 8.8 of \cite{awodey2006category}.
\end{proof}
\todo[inline]{Are we using the Yoneda lemma or the Yoneda reduction? Does it matter? Do we need references for this?}
\todo[inline]{We are again using proposition 8.8 of \cite{awodey2006category} which isn't proven in the book. I forgot if this was a problem or not.}
\begin{theorem} \label{finite-pcs-compact}
The finite colimit of compact precubical sets is compact.
\end{theorem}
\begin{proof}
From proposition 1.3 of \cite{adamek_rosicky_1994}.
\end{proof}
\begin{theorem}
Every finite precubical set is compact.
\end{theorem}
\begin{proof}
This follows from theorem \ref{finite-pcs-compact} and the density theorem.
\end{proof}
\begin{theorem} \label{pcs-filtered-colimit-finite-pcs}
Every precubical set can be canonically expressed as the filtered colimit of finite precubical sets.
\end{theorem}
\begin{proof}
\todo[inline]{Sketch of the proof. In the thesis we used something similar with precubical subsets, but I think this version will be a little cleaner and overall shorter (if it works).}
Let $X$ be a precubical set and let $\text{el}(X)$ be the category of elements of $X$.
\begin{enumerate}
    \item Every finite full subcategory of $\text{el}(X)$ forms a diagram (like with the density theorem).
    \item Let $Q(X)$ be the category of finite full subcategories of $\text{el}(X)$ with the morphisms being the inclusion maps. Then $Q(X)$ is a filtered diagram.
    \item Let $F:Q(X)\to\presheaf{\Cube}$ be the diagram where for each $S\in Q(X)$ the precubical set $F(S)$ is the colimit of the diagram $S\to\presheaf{\Cube}$. The precubical maps $F(f):F\left(S_1\right)\to F\left(S_2\right)$ are well defined (if I'm right then $F\left(S_2\right)$ is a cocone of the diagram of $F\left(S_1\right)$, which would give us a unique precubical map $F\left(S_1\right)\to F\left(S_2\right)$).
    \item For each $S\in Q(X)$ there exists a canonical precubical map $\phi(S):F(S)\to X$ (again, $X$ should be a cocone of the diagram of $F(S)$).
    \item These precubical maps make $(X,\phi)$ a cocone of $F$.
    \item $(X,\phi)$ is a (filtered) colimit of $F$.
\end{enumerate}
\todo[inline]{Terminology is a bit confusing right now. Also I think there is a good chance someone else has proven (a stronger version of) this already, which means we could use a reference instead.}
\end{proof}
\begin{theorem}
Every compact precubical set is finite.
\end{theorem}
\begin{proof}
Let $X$ be a compact precubical set and let $F:D\to\presheaf{\Cube}$ be the filtered diagram as described in theorem \ref{pcs-filtered-colimit-finite-pcs} of which $(X,\phi)$ is a filtered colimit. Then we have
\[
\colim_{d\in D}\text{Hom}\left(X,F(d)\right)\cong\text{Hom}\left(X,\colim_{d\in D}F(d)\right)\cong\text{Hom}\left(X,X\right)
\]
Let $U:\colim_{d\in D}\text{Hom}\left(X,F(d)\right)\to \text{Hom}\left(X,X\right)$ be the canonical isomorphism. For each $d\in D$ we have the morphism $\text{Hom}\left(X,\phi_d\right):\text{Hom}\left(X,F(d)\right)\to\text{Hom}\left(X,X\right)$ and let $\Phi_d:\text{Hom}\left(X,F(d)\right)\to\colim_{d\in D}\text{Hom}\left(X,F(d)\right)$ be the injection morphism of the filtered colimit $\colim_{d\in D}\text{Hom}\left(X,F(d)\right)$. By definition for all 
$d\in D$ we have $U\circ\Phi_d=\text{Hom}\left(X,\phi_d\right)$.

We have $\text{id}_X\in\text{Hom}\left(X,X\right)$ and therefore $U^{-1}\circ\text{id}_X\in \colim_{d\in D}\text{Hom}\left(X,F(d)\right)$. Then by definition of the filtered colimit of sets 
there exists a $d\in D$ and a $f\in\text{Hom}\left(X,F(d)\right)$ such that $\Phi_d\circ f=U^{-1}\circ \text{id}_X$, or in other words $\text{id}_X=U\circ\Phi_d\circ f=\text{Hom}\left(X,\phi_d\right)(f)=\phi_d\circ 
f$. This means that the identity of $X$ factors through some finite precubical set $F(d)$. Because $\text{id}_X$ is surjective this means that $\phi_d:F(d)\to X$ must be surjective as well. Since $F(d)$ is a finite precubical set $X$ must be finite as well.
\end{proof}
\todo[inline]{This proof should be correct but might be a little messy, we use a few things of which we don't explain why they are true or how we got them. However they might be trivial enough for this to not be necessary.}
\begin{theorem}
Every HDA can be canonically expressed as the filtered colimit of finite HDA.
\end{theorem}
\begin{proof}
Let $X$ be the HDA $\HDATup{X}$. Theorem \ref{pcs-filtered-colimit-finite-pcs} gives us that the precubical set $\forget\circ X$ can be expressed as the colimit of a filtered diagram of finite precubical sets. Let $F:D\to\presheaf{\Cube}$ be this diagram and let $(Y,\psi)$ be the colimit with $Y=\forget\circ X$.
\begin{enumerate}
    \item Define the diagram of HDA $G:D\to\HDA$ with $G(d)=F(d)$ and
    \[
    x\in\sCells{G(d)}\iff \psi(d)[U](x)\in\sCells{X}
    \]
    \[
    x\in\aCells{G(d)}\iff \psi(d)[U](x)\in\aCells{X}
    \]
    or something like this.
    \item Show that $(X,\phi)$ is a cocone of this diagram.
    \item Let $(Z,\theta)$ be the colimit of this diagram. There exists a unique HDA map $q:Z\to X$ with certain properties.
    \item Because we have $\forget\circ X=Y\cong\forget\circ Z$ (since the functor $\forget$ has a right adjoint it preserves colimits) $\forget\circ X$ is a colimit of $F$ as well and there exists a precubical map $q^{-1}:X\to Z$.
    \item Show that by definition this map preserves initial and final cells.
\end{enumerate}
\todo[inline]{We can use the construction in theorem \ref{HDA-cocomplete}. Given a HDA we can convert it to a precubical set. Then theorem \ref{pcs-filtered-colimit-finite-pcs} gives us a filtered diagram of finite precubical sets of which this precubical set is the colimit. Then we can convert this diagram to a diagram of finite HDA, of which the original HDA is a colimit.}
\end{proof}
\begin{theorem}
A HDA is compact if and only if it is finite.
\end{theorem}
\begin{proof}
\todo[inline]{Compact implying finite can be proven similarly to how it was proven in theorem 2.40 of the thesis. Finite implying compact is significantly more difficult (also due to the previous theorem gives us that compact implies finite as well). We might need to understand everything in the definition of compactness a little better. We need to show that if a precubical map $\colim_{d\in D}\text{Hom}\left(X,F(d)\right)$ does not preserve initial and/or final cells then the equivalent precubical map in $\text{Hom}\left(X,\colim_{d\in D}F(d)\right)$ doesn't either and vice versa.}
\end{proof}
\begin{theorem}
The category of HDA is locally finitely presentable.
\end{theorem}
\begin{proof}
\todo[inline]{Prove the statement. Note that we have already proven that $\presheaf{\Cube}$ is locally finitely presentable (theorem \ref{pcs-lfp}) and that $\HDA$ is cocomplete (theorem \ref{HDA-cocomplete}). We need to prove that the full subcategory of $\HDA$ consisting of the compact HDA is essentially small and that any HDA is a filtered colimit of the canonical diagram of compact HDA.}
\end{proof}
\begin{theorem} \label{compact-pcs-HDA}
\todo[inline]{A HDA $X$ is compact as a HDA if and only if it is compact as a precubical set.}
\end{theorem}
\todo[inline]{We need to state somewhere that precubical sets being finite is not equivalent to them being finite presheaves (a finite precubical set is a finite presheaf but there are precubical sets that are also finite presheaves but not finite precubical sets).}

\subsection{Process Replication as Rational HDA}
\label{sec:replication}

\begin{definition}
\todo[inline]{The parallel kleene star on languages of HDA $L(X)^{(*)}$ is equivalent to the operation on HDA:
\[
\coprod_{n\in\mathbb{N}}X_n\text{, }X_n=X_{n-1}\otimes X
\]
where $X_0$ is the zero-dimensional HDA with only a single node. Note that the above can trivially be expressed as a discrete diagram of HDA and its colimit.}
\end{definition}

\todo[inline]{Question to us: Can we define rational HDA as locally finite and get those as
  (filtered) colimits?}

\todo[inline]{Give examples of construction. For example the repetition of a replication of
  parallel actions like $(!(a \mid b))^{*}$.

  How does interleaving work as operation on HDA?}

\todo[inline]{According to Wikipedia in a locally finite category each morphism can be written in only finitely many ways as the composition of two non-identity morphisms. A locally finite HDA would then be one where each face map can be written in only finitely many ways as the composition of two non-identity face maps.

This is equivalent to all elements being of finite dimension. It is clear why all elements being of finite dimension implies local finity; for each of these elements there is by definition only a finite amount of face maps they are the source of. If we have an element of infinite dimension even if it can only reach a finite amount of elements (with its face maps) it will still by definition have an infinite amount of face maps breaking the local finity.

This is most likely false: "The locally finite HDA are exactly the filtered colimits of diagrams $F:D\to\HDA$ of finite HDA such that there exists a $n\in\mathbb{N}$ such that for all $d\in D$ we have $\text{dim}\left(F(d)\right)\leq n$". Instead I think it should just be that for all $d\in D$ the HDA $F(d)$ has finite dimension, which means that locally finite HDA are closed under colimits (and a colimit of HDA is locally finite if and only if every HDA in the diagram is locally finite). I'll confirm this later.}

\todo[inline]{Note that this definition of local finity is different than saying that each state (of arbitrary dimension) is directly attached to only a finite amount of other states (in other words: is the target of only a finite amount of face maps). Alternatively for all $U\in\Cube$ and $x\in X[U]$:
\[
\left|\bigsqcup_{V\in\Cube\text{, }y\in X[V]}\text{Hom}\left(y,x\right)\right|<\infty
\]
It is clear that every finite HDA is locally finite (by this definition). Not every infinite HDA is locally finite, but infinite HDA that are locally finite do exist. Every coproduct of locally finite HDA is locally finite. What condition makes a finite HDA locally finite isn't immediately obvious.

Let $F:D\to\HDA$ be a diagram of locally finite HDA with the colimit $\left(X,\phi\right)$.

If $D$ is locally finite then $X$ can still be not locally finite. For example: think of a diagram with an infinite amount of one dimensional "line" HDA $Y_n$, one zero dimensional HDA $X$ consisting of a single node and an infinite amount of HDA maps $f_n:X\to Y_n$ sending the single node in $X$ to the starting node in each $Y_n$. The colimit of this diagram is a star with infinite points that is not locally finite.

Suppose that for all $d\in D$ both $\text{Hom}\left(F(d),-\right)$ and $\text{Hom}\left(-,F(d)\right)$ are finite. Then $X$ is most likely locally finite... however this condition does exclude some filtered diagrams that do generate locally finite colimits...

I'm not sure if we're actually using this definition, so for now I'm leaving it at this.}

\todo[inline]{Originally I thought that in neither definition of locally finite HDA is local finity closed under the parallel kleene star (nor do finite HDA always generate locally finite HDA). For the first definition this is because (I thought) we can end up with element of infinite dimension. For the second definition the problem can be seen with the parallel kleene star of the one-dimensional "line" HDA. However these cases are I think still locally finite. In the first case we don't actually have elements of infinite dimension, instead we have elements of arbitrary dimension which should be fine. Something similar is true for the second case: No element is connected to an infinite amount of other elements, only an arbitrary amount of other elements. I however haven't been able to confirm yet if in these definitions for local finity the locally finite HDA are closed under the parallel kleene star.}

\begin{definition}
The interleaving of HDA is defined as the following: Let $X$ and $Y$ be HDA. For all $U,V,W\in\Cube$, $x\in X[V]$, $y\in Y[W]$ and $A,B\subseteq U$ we define
\[
\left(X\diamond Y\right)[U]=\left(X[U]\times Y[\varepsilon]\right)\cup\left(X[\varepsilon]\times Y[U]\right)\text{, }\quad\delta_{A,B}(x, y)=\left(\delta_{A\cap V,B\cap V}(x),\delta_{A\cap W,B\cap W}(y)\right)
\]
and $\left(X\diamond Y\right)_{\bot}=\left(\sCells{X}\times Y[\varepsilon]\right)\cup\left(X[\varepsilon]\times\sCells{Y}\right)$, $\left(X\diamond Y\right)^{\top}=\left(\aCells{X}\times Y[\varepsilon]\right)\cup\left(X[\varepsilon]\times\aCells{Y}\right)$.
\todo[inline]{I didn't know what symbol to use so I went with $\diamond$.}
\todo[inline]{At the moment I don't really know how to explain why the interleaving can be defined like this, I hope this definition is somewhat clear.}
\todo[inline]{We might need to define how the interleaving operation interacts with colimits and languages.}
\end{definition}

\begin{definition}
A subcategory $D$ of $C$ is called a target-closed subcategory if it is full and for all $d\in\text{obj}(D)$ and all $c\in\text{obj}(C)$ if $\text{Hom}_C(c,d)\not=\emptyset$ then $c\in\text{obj}(D)$.
\end{definition}
\todo[inline]{I made \textit{"target-closed subcategory"} up, since I don't know if there exists a proper term for it.}
\todo[inline]{Do we need the stuff about the category of elements? Or can we do without? The question is then what we use for our filtered category $D$.}
Let $\text{el}(X)$ be the category of elements of a precubical set or HDA $X$. Its objects are pairs $(U,x)$ with $U\in\text{obj}(\Cube)$ and $x\in X[U]$. Its morphisms $(U,x)\to(V,y)$ are coface maps $d:U\to V$ in $\Cube$ such that $X_f(y)=x$. A precubical set or HDA is finite if and only if its category of elements is finite.
\todo[inline]{Does this make sense?}
\begin{lemma}
Let $X$ be a precubical set. Every precubical subset of $X$ can be uniquely identified with a target-closed subcategory of $\text{el}(X)$ and every target-closed subcategory of $\text{el}(X)$ corresponds uniquely to a precubical subset of $X$.
\end{lemma}
\begin{proof}
\todo[inline]{Prove the statement.}
\end{proof}
\todo[inline]{The reason why we talk about these categories of elements and target-closed subcategories is because we want to find a filtered category $D$ that makes a diagram $F:D\to\HDA$ such that for each $d\in D$ the HDA $F(d)$ is a finite sub-HDA of $X$ and such that the HDA maps $F(f)$ are the inclusion maps.}
